Probabilistic Graphical Models on Multi-Core CPUs using Java 8

In this paper, we discuss software design issues related to the development of parallel computational intelligence algorithms on multi-core CPUs, using the new Java 8 functional programming features. In particular, we focus on probabilistic graphical models (PGMs) and present the parallelisation of a collection of algorithms that deal with inference and learning of PGMs from data. Namely, maximum likelihood estimation, importance sampling, and greedy search for solving combinatorial optimisation problems. Through these concrete examples, we tackle the problem of defining efficient data structures for PGMs and parallel processing of same-size batches of data sets using Java 8 features. We also provide straightforward techniques to code parallel algorithms that seamlessly exploit multi-core processors. The experimental analysis, carried out using our open source AMIDST (Analysis of MassIve Data STreams) Java toolbox, shows the merits of the proposed solutions.

==> hl_short.tex <==
\usepackage{xspace}
\usepackage{graphics,graphicx,epsfig}
\usepackage{url}

\newcommand{\nc}{\newcommand}

%      HELGE's EGNE "NEWCOMMANDS"



%%      THEOREMER OG SLIKT%
%
\newtheorem{hl_example}{Example}
\newtheorem{hl_algorithm}{Algorithm}
\newtheorem{hl_theorem}{Theorem}
\newtheorem{hl_proposition}{Proposition}
\newtheorem{hl_lemma}{Lemma}
\newtheorem{hl_corollary}{Corollary}
\newtheorem{hl_definition}{Definition}
\newtheorem{hl_conjecture}{Conjecture}
\newenvironment{hl_nonumberenv}[1]{{\bf #1}\begin{it}}{\end{it}}
\newtheorem{hl_proof}{Proof}



%      KOMMENTARMARKERING

\nc{\vekk}[1]{}   %         \vekk{Brukes for å markere vekk tekst}
%\nc{\comment}[1]{\mbox{}\marginpar{\raggedright\hspace{0pt}#1}}%
\nc{\hl}[1]{\comment{{\bf HL:} #1}} %
\nc{\tdn}[1]{\comment{{\bf TDN:} #1}} %



%      BEGIN/END

\nc{\bex}{\begin{example}} \nc{\eex}{\end{example}}

%\nc{\bth}{\begin{theorem}}
%\nc{\eth}{\end{theorem}}

\nc{\ble}{\begin{lemma}}
\nc{\ele}{\end{lemma}}

\nc{\bco}{\begin{conjecture}}
\nc{\eco}{\end{conjecture}}

\nc{\beq}{\begin{equation}}
\nc{\eeq}{\end{equation}}

\nc{\beqa}{\begin{eqnarray}}
\nc{\eeqa}{\end{eqnarray}}

\nc{\beqas}{\begin{eqnarray*}}%
\nc{\eeqas}{\end{eqnarray*}}

\nc{\bsp}{\[\begin{array}{rcl}}
\nc{\esp}{\end{array}\]}

\nc{\btab}[1]{\begin{tabular}{#1}}
\nc{\etab}{\end{tabular}}

\nc{\bfi}{\begin{figure}[htpb]}
\nc{\efi}{\end{figure}}

\nc{\ben}{\begin{enumerate}}
\nc{\een}{\end{enumerate}}

\nc{\bit}{\begin{itemize}}
\nc{\eit}{\end{itemize}}

\nc{\bde}{\begin{description}}
\nc{\ede}{\end{description}}


%      PRODUKT, BINOMISKE TING OG SUMMER

\nc{\pin}{\prod_{i=1}^n} \nc{\pjm}{\prod_{j=1}^m}
\nc{\pkm}{\prod_{k=1}^m} \nc{\pjM}{\prod_{j=1}^M}
\nc{\suin}{\sum_{i=1}^n} \nc{\sujm}{\sum_{j=1}^m}
\nc{\sukm}{\sum_{k=1}^m} \nc{\sujM}{\sum_{j=1}^M} \nc{\bimr}{\left
(_r^m \right)} \nc{\birs}{\left (_s^r \right)}
\nc{\bin}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      CAL-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\nc{\cal}{\mathcal}

\nc{\calDelta}{\mbox{$\cal{\Delta}$}}

% \nc{\calA}{\mbox{${\cal A}$}} \nc{\calB}{\mbox{$\cal{B}$}}
% \nc{\calC}{\mbox{$\cal{C}$}} \nc{\calD}{\mbox{$\cal{D}$}}
% \nc{\calE}{\mbox{$\cal{E}$}} \nc{\calF}{\mbox{$\cal{F}$}}
% \nc{\calG}{\mbox{$\cal{G}$}} \nc{\calH}{\mbox{$\cal{H}$}}
% \nc{\calI}{\mbox{$\cal{I}$}} \nc{\calJ}{\mbox{$\cal{J}$}}
% \nc{\calK}{\mbox{$\cal{K}$}} \nc{\calL}{\mbox{$\cal{L}$}}
% \nc{\calM}{\mbox{$\cal{M}$}} \nc{\calN}{\mbox{$\cal{N}$}}
% \nc{\calO}{\mbox{$\cal{O}$}} \nc{\calP}{\mbox{$\cal{P}$}}
% \nc{\calQ}{\mbox{$\cal{Q}$}} \nc{\calR}{\mbox{$\cal{R}$}}
% \nc{\calS}{\mbox{$\cal{S}$}} \nc{\calT}{\mbox{$\cal{T}$}}
% \nc{\calU}{\mbox{$\cal{U}$}} \nc{\calV}{\mbox{$\cal{V}$}}
% \nc{\calW}{\mbox{$\cal{W}$}} \nc{\calX}{\mbox{$\cal{X}$}}
% \nc{\calY}{\mbox{$\cal{Y}$}} \nc{\calZ}{\mbox{$\cal{Z}$}}
% \nc{\calz}{\mbox{$\cal{z}$}}



\nc{\calA}{{\ensuremath{\cal{A}}}} \nc{\calB}{{\ensuremath{\cal{B}}}}
\nc{\calC}{{\ensuremath{\cal{C}}}} \nc{\calD}{{\ensuremath{\cal{D}}}}
\nc{\calE}{{\ensuremath{\cal{E}}}} \nc{\calF}{{\ensuremath{\cal{F}}}}
\nc{\calG}{{\ensuremath{\cal{G}}}} \nc{\calH}{{\ensuremath{\cal{H}}}}
\nc{\calI}{{\ensuremath{\cal{I}}}} \nc{\calJ}{{\ensuremath{\cal{J}}}}
\nc{\calK}{{\ensuremath{\cal{K}}}} \nc{\calL}{{\ensuremath{\cal{L}}}}
\nc{\calM}{{\ensuremath{\cal{M}}}} \nc{\calN}{{\ensuremath{\cal{N}}}}
\nc{\calO}{{\ensuremath{\cal{O}}}} \nc{\calP}{{\ensuremath{\cal{P}}}}
\nc{\calQ}{{\ensuremath{\cal{Q}}}} \nc{\calR}{{\ensuremath{\cal{R}}}}
\nc{\calS}{{\ensuremath{\cal{S}}}} \nc{\calT}{{\ensuremath{\cal{T}}}}
\nc{\calU}{{\ensuremath{\cal{U}}}} \nc{\calV}{{\ensuremath{\cal{V}}}}
\nc{\calW}{{\ensuremath{\cal{W}}}} \nc{\calX}{{\ensuremath{\cal{X}}}}
\nc{\calY}{{\ensuremath{\cal{Y}}}} \nc{\calZ}{{\ensuremath{\cal{Z}}}}
\nc{\calz}{{\ensuremath{\cal{z}}}}



%\nc{\NP}{\mbox{$\calN\calP$}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      BOLDMATH-TING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\nc{\bm}{\boldmath}
% \nc{\bm}{\bf}
\nc{\bma}{{\ensuremath{\boldsymbol{a}}}} 
\nc{\bmb}{{\ensuremath{\boldsymbol{b}}}}
\nc{\bmc}{{\ensuremath{\boldsymbol{c}}}} \nc{\bmd}{{\ensuremath{\boldsymbol{d}}}}
\nc{\bme}{{\ensuremath{\boldsymbol{e}}}} \nc{\bmf}{{\ensuremath{\boldsymbol{f}}}}
\nc{\bmg}{{\ensuremath{\boldsymbol{g}}}} \nc{\bmh}{{\ensuremath{\boldsymbol{h}}}}
\nc{\bmi}{{\ensuremath{\boldsymbol{i}}}} \nc{\bmj}{{\ensuremath{\boldsymbol{j}}}}
\nc{\bmk}{{\ensuremath{\boldsymbol{k}}}} \nc{\bml}{{\ensuremath{\boldsymbol{l}}}}
\nc{\bmm}{{\ensuremath{\boldsymbol{m}}}} \nc{\bmn}{{\ensuremath{\boldsymbol{n}}}}
\nc{\bmo}{{\ensuremath{\boldsymbol{o}}}} \nc{\bmp}{{\ensuremath{\boldsymbol{p}}}}
\nc{\bmq}{{\ensuremath{\boldsymbol{q}}}} \nc{\bmr}{{\ensuremath{\boldsymbol{r}}}}
\nc{\bms}{{\ensuremath{\boldsymbol{s}}}} \nc{\bmt}{{\ensuremath{\boldsymbol{t}}}}
\nc{\bmu}{{\ensuremath{\boldsymbol{u}}}} \nc{\bmv}{{\ensuremath{\boldsymbol{v}}}}
\nc{\bmw}{{\ensuremath{\boldsymbol{w}}}} \nc{\bmx}{{\ensuremath{\boldsymbol{x}}}}
\nc{\bmy}{{\ensuremath{\boldsymbol{y}}}} \nc{\bmz}{{\ensuremath{\boldsymbol{z}}}}

% \nc{\bma}{{\mbox{\bm $a$}}} 
% \nc{\bmb}{{\mbox{\bm $b$}}}
% \nc{\bmc}{{\mbox{\bm $c$}}} \nc{\bmd}{{\mbox{\bm $d$}}}
% \nc{\bme}{{\mbox{\bm $e$}}} \nc{\bmf}{{\mbox{\bm $f$}}}
% \nc{\bmg}{{\mbox{\bm $g$}}} \nc{\bmh}{{\mbox{\bm $h$}}}
% \nc{\bmi}{{\mbox{\bm $i$}}} \nc{\bmj}{{\mbox{\bm $j$}}}
% \nc{\bmk}{{\mbox{\bm $k$}}} \nc{\bml}{{\mbox{\bm $l$}}}
% \nc{\bmm}{{\mbox{\bm $m$}}} \nc{\bmn}{{\mbox{\bm $n$}}}
% \nc{\bmo}{{\mbox{\bm $o$}}} \nc{\bmp}{{\mbox{\bm $p$}}}
% \nc{\bmq}{{\mbox{\bm $q$}}} \nc{\bmr}{{\mbox{\bm $r$}}}
% \nc{\bms}{{\mbox{\bm $s$}}} \nc{\bmt}{{\mbox{\bm $t$}}}
% \nc{\bmu}{{\mbox{\bm $u$}}} \nc{\bmv}{{\mbox{\bm $v$}}}
% \nc{\bmw}{{\mbox{\bm $w$}}} \nc{\bmx}{{\mbox{\bm $x$}}}
% \nc{\bmy}{{\mbox{\bm $y$}}} \nc{\bmz}{{\mbox{\bm $z$}}}


\nc{\bmA}{{\ensuremath{\boldsymbol{A}}}} \nc{\bmB}{{\ensuremath{\boldsymbol{B}}}}
\nc{\bmC}{{\ensuremath{\boldsymbol{C}}}} \nc{\bmD}{{\ensuremath{\boldsymbol{D}}}}
\nc{\bmE}{{\ensuremath{\boldsymbol{E}}}} \nc{\bmF}{{\ensuremath{\boldsymbol{F}}}}
\nc{\bmG}{{\ensuremath{\boldsymbol{G}}}} \nc{\bmH}{{\ensuremath{\boldsymbol{H}}}}
\nc{\bmI}{{\ensuremath{\boldsymbol{I}}}} \nc{\bmJ}{{\ensuremath{\boldsymbol{J}}}}
\nc{\bmK}{{\ensuremath{\boldsymbol{K}}}} \nc{\bmL}{{\ensuremath{\boldsymbol{L}}}}
\nc{\bmM}{{\ensuremath{\boldsymbol{M}}}} \nc{\bmN}{{\ensuremath{\boldsymbol{N}}}}
\nc{\bmO}{{\ensuremath{\boldsymbol{O}}}} \nc{\bmP}{{\ensuremath{\boldsymbol{P}}}}
\nc{\bmQ}{{\ensuremath{\boldsymbol{Q}}}} \nc{\bmR}{{\ensuremath{\boldsymbol{R}}}}
\nc{\bmS}{{\ensuremath{\boldsymbol{S}}}} \nc{\bmT}{{\ensuremath{\boldsymbol{T}}}}
\nc{\bmU}{{\ensuremath{\boldsymbol{U}}}} \nc{\bmV}{{\ensuremath{\boldsymbol{V}}}}
\nc{\bmW}{{\ensuremath{\boldsymbol{W}}}} \nc{\bmX}{{\ensuremath{\boldsymbol{X}}}}
\nc{\bmY}{{\ensuremath{\boldsymbol{Y}}}} \nc{\bmZ}{{\ensuremath{\boldsymbol{Z}}}}

% \nc{\bmA}{{\mbox{\bm $A$}}} \nc{\bmB}{{\mbox{\bm $B$}}}
% \nc{\bmC}{{\mbox{\bm $C$}}} \nc{\bmD}{{\mbox{\bm $D$}}}
% \nc{\bmE}{{\mbox{\bm $E$}}} \nc{\bmF}{{\mbox{\bm $F$}}}
% \nc{\bmG}{{\mbox{\bm $G$}}} \nc{\bmH}{{\mbox{\bm $H$}}}
% \nc{\bmI}{{\mbox{\bm $I$}}} \nc{\bmJ}{{\mbox{\bm $J$}}}
% \nc{\bmK}{{\mbox{\bm $K$}}} \nc{\bmL}{{\mbox{\bm $L$}}}
% \nc{\bmM}{{\mbox{\bm $M$}}} \nc{\bmN}{{\mbox{\bm $N$}}}
% \nc{\bmO}{{\mbox{\bm $O$}}} \nc{\bmP}{{\mbox{\bm $P$}}}
% \nc{\bmQ}{{\mbox{\bm $Q$}}} \nc{\bmR}{{\mbox{\bm $R$}}}
% \nc{\bmS}{{\mbox{\bm $S$}}} \nc{\bmT}{{\mbox{\bm $T$}}}
% \nc{\bmU}{{\mbox{\bm $U$}}} \nc{\bmV}{{\mbox{\bm $V$}}}
% \nc{\bmW}{{\mbox{\bm $W$}}} \nc{\bmX}{{\mbox{\bm $X$}}}
% \nc{\bmY}{{\mbox{\bm $Y$}}} \nc{\bmZ}{{\mbox{\bm $Z$}}}




\nc{\bmUpsilon}{{\mbox{\bm $\Upsilon$}}}
\nc{\bmupsilon}{{\mbox{\bm $\upsilon$}}}
\nc{\bmalpha}{{\mbox{\bm $\alpha$}}}
\nc{\bmbeta}{{\mbox{\bm $\beta$}}}
\nc{\bmgamma}{{\mbox{\bm $\gamma$}}}
\nc{\bmGamma}{{\mbox{\bm $\Gamma$}}}
\nc{\bmdelta}{{\mbox{\bm $\delta$}}}
\nc{\bmDelta}{{\mbox{\bm $\Delta$}}}
\nc{\bmeps}{{\mbox{\bm $\epsilon$}}}
\nc{\bmepsilon}{\bmeps}
\nc{\bmphi}{{\mbox{\bm $\phi$}}}
\nc{\bmPhi}{{\mbox{\bm $\Phi$}}}
\nc{\bmlambda}{{\mbox{\bm $\lambda$}}}
\nc{\bmLambda}{{\mbox{\bm $\Lambda$}}}
\nc{\bmmu}{{\mbox{\bm $\mu$}}}
\nc{\bmnu}{{\mbox{\bm $\nu$}}}
\nc{\bmpi}{{\mbox{\bm $\pi$}}}
\nc{\bmrho}{{\mbox{\bm$\rho$}}}
\nc{\bmpsi}{{\mbox{\bm $\psi$}}}
\nc{\bmPsi}{{\mbox{\bm $\Psi$}}}
\nc{\bmsigma}{{\mbox{\bm $\sigma$}}}
\nc{\bmSigma}{{\mbox{\bm $\Sigma$}}}
\nc{\bmtheta}{{\mbox{\bm $\theta$}}}
\nc{\bmTheta}{{\mbox{\bm $\Theta$}}}
\nc{\bmeta}{{\mbox{\bm $\eta$}}}
\nc{\bmzeta}{{\mbox{\bm $\zeta$}}}
\nc{\bmxi}{{\mbox{\bm $\xi$}}} \nc{\bmXi}{{\mbox{\bm $\Xi$}}}
\nc{\bmnabla}{{\mbox{\bm $\nabla$}}}
\nc{\bmomega}{{\mbox{\bm $\omega$}}}
\nc{\bmOmega}{{\mbox{\bm $\Omega$}}}

\nc{\bmen}{{\bf 1}} \nc{\bmhalf}{{\bf\frac{1}{2}}}
\nc{\bmnull}{{\bf \ensuremath{0}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% General terminology
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\Var}{\mbox{Var}} \nc{\Cov}{\mbox{Cov}}
\nc{\E}{\mbox{$\mathbb{E}$}}
\nc{\KL}[2]{D\left(\,#1\,\norm\,#2\,\right)}
\nc{\convL}{\stackrel{\calL}{\rightarrow}} \nc{\given}{|}
%\nc{\norm}{||}
\nc{\norm}{\|} \nc{\sizeof}[1]{\left|#1\right|}

\nc{\iffp}{\mbox{$\Leftrightarrow$}} \nc{\ien}{\mbox{$i=1\ld n$}}
%\nc{\R}{\mbox{$\mathbb{R}$}}
\nc{\nat}{\mbox{$\mathbb{N}$}} \nc{\infinity}{\infty}
\nc{\ld}{,\ldots,} \nc{\defi}{:=} \nc{\incl}{\subset}
\nc{\upin}[2]{#1^{(#2)}} \nc{\non}{\nonumber}
\nc{\stless}{\stackrel{\mbox{st}}{\leq}}
\gdef\qed{\relax\ifmmode~\hfill\square\else\unskip\nobreak
    ~\hfill$\square$\fi}
\nc{\boxen}{\begin{flushright}$\rule{3mm}{3mm}$\end{flushright}}
\newcommand{\trans}{^{\mbox{\tiny{T}}}}
%\newcommand{\trans}{\top}
\newcommand{\T}{\trans}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special reliability analysis
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nc{\h}{\mbox{$h(\bmp)$}}
\nc{\hm}{\mbox{$h^m(\bmp)$}}
\nc{\hnei}{\mbox{$h({\bf p})$}}
\nc{\hmnei}{\mbox{$h^m({\bf p})$}}
\nc{\hj}{h_j(\bmp)}
\nc{\hmj}{h_j^m(\bmp)}
\nc{\hjm}{\hmj}
\nc{\ph}{\phi(\bmx)}
\nc{\Ph}{\phi(\bmX)}
%\nc{\p}{\overline P}
\nc{\ip}{\coprod}
\nc{\phd}{\phi^D (\bmx)}
\nc{\Phd}{\phi^D(\bmX)}
\nc{\hd}{h^D (\bmp)}
\nc{\hdm}{\left( h^D (\bmp) \right)^m}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% BN related stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \nc{\pa}[1]{{\rm pa}\left(#1\right)}
 \nc{\mb}[1]{{\rm mb}\left(#1\right)}
 \nc{\sspace}[1]{\ensuremath{sp\left(#1\right)}}
% \nc{\sspace}[1]{{\rm sp}\left(#1\right)}
 \nc{\child}[1]{\mbox{${\rm ch}\left(#1\right)$}}
 \nc{\indep}{\mbox{$\perp\!\!\!\perp$}}
 \nc{\nonindep}{\not\!\!\!\indep} \nc{\NB}{Na\"{\i}ve Bayes\xspace}
 \nc{\nB}{na\"{\i}ve Bayes\xspace}
 \nc{\MDL}{\mbox{MDL}\xspace} \nc{\MDLp}{$\mbox{MDL}_p$\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This part here for the HuginToPsTrics stuff by Thomas
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Fbox}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\parbox[c][#1]{#1}{\centerline{#5}}}}}}
\newcommand{\Fnode}[5][0.5cm]{\cnodeput[doubleline=false](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\FDblnode}[5][0.5cm]{\cnodeput[doubleline=true](#2,#3){#4}{\makebox[#1]{#5}}}
\newcommand{\Fdiam}[5][0.3cm]{\rput(#2,#3){\dianode{#4}{\makebox[#1]{#5}}}}
\newcommand{\Fovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode{#4}{\makebox[#1]{#5}}}}
\newcommand{\FDblovalnode}[5][0.5cm]{\rput(#2,#3){\ovalnode[doubleline=true]{#4}{\makebox[#1]{#5}}}}
\newcommand{\Frect}[5][0.5cm]{\rput(#2,#3){\rnode{#4}{\psframebox{\makebox[#1]{#5}}}}}
\newcommand{\arc}[3][solid]{\ncline[linestyle=#1]{->}{#2}{#3}}
%\newpsobject{showgrid}{psgrid}{subgriddiv=1,griddots=10,gridlabels=6pt}
%\psset{unit=0.5cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% pstexfig: Latex-type figures from xfig.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\pstexfig}[2] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}

\newcommand{\pstexFig}[2] {
\begin{nopagebreak}
  \begin{figure*}[htbp]
    \begin{center}
      \input{./FIGS/#1.pstex_t}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure*}
\end{nopagebreak}
}

\newcommand{\pstexfigSlide}[1] {
\begin{nopagebreak}
    \begin{center}
        \input{./#1.pstex_t}
    \end{center}
\end{nopagebreak}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% epsfigur: Get an eps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\epsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \epsfig{file =./FIGS/#1.eps,width=#3mm}
        \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% psfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\psfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm,angle=-90}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rpsfigur: Get an ps-fig from file
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Rpsfigur}[3] {
\begin{nopagebreak}
  \begin{figure}[htpb]
    \begin{center}
      \psfig{file =./FIGS/#1.ps,width=#3mm}
       \caption{#2}
      \label{fig:#1}
    \end{center}
  \end{figure}
\end{nopagebreak}
}



\nc{\figref}[1]{\figurename~\ref{fig:#1}\xspace}
\nc{\tabref}[1]{Table~\ref{tab:#1}\xspace}
\nc{\equref}[1]{Equation~(\ref{equ:#1})\xspace}
\nc{\secref}[1]{Section~\ref{sec:#1}\xspace}
\nc{\algoref}[1]{Algorithm~\ref{algo:#1}\xspace}
\nc{\stepref}[1]{Step~\ref{step:#1}\xspace}

\nc{\includebib}{\bibliography{defs,%
                               hl,%
                               master,%
                               dynamic,%
                               reliability,%
                               troubleshoot,%
                               class,%
                               learning,%
                               luigi,%
			      footy,%
                               antonio,%
%                               mte,%
                               global%
}}

